A Survey On Text-to-3D Contents Generation In The Wild

3D content creation plays a vital role in various applications, such as gaming, robotics simulation, and virtual reality. However, the process is labor-intensive and time-consuming, requiring skilled designers to invest considerable effort in creating a single 3D asset. To address this challenge, text-to-3D generation technologies have emerged as a promising solution for automating 3D creation. Leveraging the success of large vision language models, these techniques aim to generate 3D content based on textual descriptions. Despite recent advancements in this area, existing solutions still face significant limitations in terms of generation quality and efficiency. In this survey, we conduct an in-depth investigation of the latest text-to-3D creation methods. We provide a comprehensive background on text-to-3D creation, including discussions on datasets employed in training and evaluation metrics used to assess the quality of generated 3D models. Then, we delve into the various 3D representations that serve as the foundation for the 3D generation process. Furthermore, we present a thorough comparison of the rapidly growing literature on generative pipelines, categorizing them into feedforward generators, optimization-based generation, and view reconstruction approaches. By examining the strengths and weaknesses of these methods, we aim to shed light on their respective capabilities and limitations. Lastly, we point out several promising avenues for future research. With this survey, we hope to inspire researchers further to explore the potential of open-vocabulary text-conditioned 3D content creation.

==> sections/05_image_generation.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{figures/3d-gan-pipeline.pdf}
    \caption{\textbf{The general pipeline of 3D-aware GAN.}
    The 3D-aware GAN framework generates 3D representations including Tri-plane~\cite{eg3d, epigraf}, Voxel~\cite{xu2021volumegan, schwarz2022voxgraf}, and Mesh~\cite{Gao2022NeurIPS}. These representations are then utilized to predict the color and density for volume rendering. The discriminator is omitted since it follows a similar approach as conventional 2D GANs.}
    \label{fig:3dgan_pipeline}
\end{figure*}


\section{Learning from 2D data}\label{sec:image_generation}
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/FLOPS-v2.pdf}
    \caption{\textbf{FID \textit{v.s.} Resolution} of representative 3D synthesis methods trained on FFHQ~\cite{stylegan}. We annotate each method by their FID score and GigaFLOPS.}
    \label{fig:flops}
\end{figure}


The goal of learning 3D representation from 2D data is mostly to explicitly control the camera viewpoint when synthesizing images \cite{shen2020interpreting, tewari2020stylerig, deng2020disentangled, yang2021semantic, leimkuhler2021freestylegan}.
Although 2D GAN-based models deliver impressive results, finding a reasonable direction in the latent space is not easy and usually cannot support full control of the rendering viewpoint.
This survey focuses on works that explicitly generate 3D representations for 3D-aware image synthesis.
In contrast to 3D data-supervised methods that are directly trained with shapes, most 2D data-based generation methods are supervised by images through differentiable neural rendering because there are few high-quality and large-scale datasets of renderable 3D representations for training generative models.
Due to the lack of renderable 3D representations, auto-encoder architectures are rarely used in this task. Instead, most methods adopt generative adversarial models, which sample a latent vector from the latent space and decode it to the target representation, as shown in \cref{fig:3dgan_pipeline}.



Similar to 3D data-based generation, there are also several 3D representations commonly used in the task of 2D data-based 3D generation. These include depth/normal maps, voxel grids, and neural fields.
Point clouds and meshes are not well explored in generative image synthesis, partly because current differentiable neural rendering cannot provide effective gradient signals to optimize these two representations easily.
The key factors to consider when incorporating 3D representation for 2D image generation are quality and efficiency, where quality includes image realism and view consistency. Representative methods that learn from 2D data are summarized in \cref{tab:representation_classification}. Additionally, \cref{fig:flops} and \cref{tab:3dimage_generation} provide properties of representative methods.


\subsection{Depth/Normal Maps}

The depth and normal maps are easily accessible representations that partially reveal the geometry of 3D scenes or objects.
Since they only show the geometry from one side, they are usually referred to as 2.5D representations.
The depth and normal maps can be easily involved in image generation (\textit{i.e.}, processed by 2D convolutional neural networks rather than 3D architectures) as they share a similar data format to 2D images.
Most methods \cite{wang2016generative, noguchi2019rgbd, shi20223d} leverage GAN models to generate depth or normal maps for 3D-aware image synthesis.

S2-GAN \cite{wang2016generative} proposes to consider the underlying 3D geometry when generating images, where it refers to the geometry as "structure" and the image as "style". It develops the Structure-GAN, which maps a sampled latent vector to a surface normal map. The normal map is then fed into the Style-GAN with another sampled latent vector to generate the image. The Structure-GAN is implemented using a set of convolution and deconvolution layers, and the Style-GAN is designed based on the conditional GAN \cite{mirza2014conditional}. By disentangling the generation of the structure and style, S2-GAN makes the generative process more interpretable and enables the controllability of image synthesis given surface normal maps.
To explicitly control the viewpoint of rendered images, RGBD-GAN \cite{noguchi2019rgbd} passes camera parameters into the generator. It assumes that RGB and depth images can be generated simultaneously and learns from 2D image data only. To ensure the inter-view consistency of synthesized images, \cite{noguchi2019rgbd} generates two RGBD images from two different viewpoints and warps the RGB-D image from one view to another to compute the consistency loss. However, the model fails to capture this relationship when the contents in the image become more complex (\textit{e.g.}, bedrooms) and outputs a flat plane.
In contrast, Wang \etal \cite{wang2016generative} and Shi \etal \cite{shi20223d} argue that appearance should be rendered conditioned on the geometry, using normal maps and depth maps, respectively.
Similar to S2-GAN \cite{wang2016generative}, DepthGAN \cite{shi20223d} develops a dual-path generator for 3D-aware image synthesis. However, in contrast to S2-GAN, which explicitly conditions image generation on the synthesized geometry, DepthGAN extracts intermediate features from the geometry path and injects them into the image path.
DepthGAN \cite{shi20223d} also designs a switchable discriminator that not only classifies the RGB-D image but also regresses from the RGB image to the depth, which is then compared with the depth from the generator.
While depth or normal maps work well with 2D GAN models, which can efficiently synthesize high-resolution images, 2D CNN-based generators do not guarantee the inter-view consistency of generated images \cite{sitzmann2019srns}, even when supervised with the view consistency loss. Moreover, depth and normal maps are 2.5D representations that cannot fully capture the geometry of the scene.


\subsection{Voxel Grids}


There are generally two ways to synthesize images from voxel grids.
The first way is to use voxel grids only to represent 3D shapes, which are then used to render depth maps to guide image generation.
The second way is to embed the geometry and appearance of scenes with voxel grids.
Inspired by the graphics rendering pipeline, Zhu \etal \cite{zhu2018visual} and Chen \etal \cite{chen2021towards} decompose the image generation task into 3D shape generation and 2D image generation. They adopt voxel grids for shape generation, followed by a projection operator that renders voxel grids into the depth map under a viewpoint. The depth map is then used as guidance for RGB image generation. Similar to S2-GAN, Zhu \etal \cite{zhu2018visual} utilize a conditional GAN to synthesize the 2D image based on the rendered depth map. To enable illumination control, Chen \etal \cite{chen2021towards} generate different image components (\textit{e.g.}, diffuse albedo, specular, and roughness) based on the rendered depth and compose the final RGB output following the physical image formation process.
On the other hand, some methods \cite{nguyen2019hologan, nguyen2020blockgan, schwarz2022voxgraf} represent the underlying geometry and appearance in voxel grids simultaneously.
HoloGAN \cite{nguyen2019hologan} leverages a 3D CNN-based generator to produce a 3D feature volume from a latent vector. A projection unit then projects the voxels to 2D features, and the subsequent 2D decoder outputs the final RGB image. To control the viewpoint, HoloGAN applies 3D transformations to voxel grids, which ensures the underlying 3D geometric property.
Based on HoloGAN, BlockGAN \cite{nguyen2020blockgan} generates multiple feature volumes, each representing a 3D entity, and composes them into a feature volume for the whole 3D scene. This strategy enables it to render images containing multiple objects.
Instead of learning a 3D feature volume, PlatonicGAN directly predicts RGB and alpha volumes \cite{Henzler2019ICCV}, but is limited to a low resolution.
More recently, VoxGRAF \cite{schwarz2022voxgraf} attempts to synthesize RGB and alpha volumes and render images from volumes through volume rendering techniques. By removing the 2D CNN renderers, VoxGRAF promises to render view-consistent images. To achieve the rendering of high-resolution images, VoxGRAF adopts sparse voxel grids to represent scenes. It first generates a low-resolution dense volume and then progressively upsamples the resolution of the volume and prunes voxels in the empty space. 

\subsection{Neural Fields}

Image synthesis methods based on neural fields generally adopt MLP networks to implicitly represent the properties of each point in the 3D space, followed by a differentiable renderer to output an image under a specific viewpoint.%
The volume renderer~\cite{volumerendering} is the most commonly used renderer for 3D-aware image synthesis.
Most of the methods use GANs to supervise the learning of neural fields.
GRAF~\cite{graf} firstly introduces the concept of generative neural radiance fields. An MLP-based generator is conditioned on a shape noise and an appearance noise and predicts the density and the color of points along each ray. Then, a volume renderer gathers the information along all rays to synthesize a 2D image. Due to the slow rendering process, a patch-based discriminator is used to differentiate between the real and fake patches instead of the complete images.
$\pi$-GAN~\cite{pigan} uses a similar setting as GRAF, but it adopts SIREN~\cite{sitzmann2020siren} rather than ReLU MLPs for representation, which is more capable of modeling fine details. It utilizes progressive training with an image-based discriminator. Besides, instead of using two latent codes, $\pi$-GAN employs a StyleGAN-like mapping network to condition the SIREN on a latent code through FiLM conditioning~\cite{perez2018film,dumoulin2018featurefilm}.
Although the above methods improve the quality of 3D-aware image synthesis significantly, they still face several challenges. First, the good quality of rendered images does not imply a decent underlying shape and guarantees inter-view consistency. Second, due to the huge number of points queried along all rays and the complex rendering process, rendering an image from the model takes a lot of time. Consequently, it is hard to train a model on high-resolution images efficiently. Third, they all assume a prior distribution of camera poses on the dataset, which may not be accurate enough.


To mitigate the first issue, ShadeGAN~\cite{shadegan} adds a lighting constraint to the generator. It generates the albedo instead of the color for each point. A shading model operates on the generated albedo map, the normal map derived from densities, the sampled camera viewpoint, and the sampled lighting source to render an RGB image.
GOF~\cite{generativeoccupancy} analyzes the weight distribution on points along a ray. The cumulative rendering process cannot ensure a low-variance distribution on rays, leading to diffuse object surfaces. While occupancy-based neural fields can satisfy the requirement, they suffer from the optimization problem that gradients only exist on surfaces. Hence, GOF unifies the two representations by gradually shrinking the sampling region to a minimal neighboring region around the surface, resulting in neat surfaces and faster training.
GRAM~\cite{gram} also examines the point sampling strategy. It claims that the deficient point sampling strategy in prior work causes the inadequate expressiveness of the generator on fine details and that the noise caused by unstable Monte Carlo sampling leads to inefficient GAN training. GRAM proposes to regulate the learning of neural fields on 2D manifolds and only optimizes the ray-manifold intersection points.
MVCGAN~\cite{zhang2022multiview} attempts to alleviate the consistency problem by adding a multi-view constraint on the generator. For the same latent code, two camera poses are sampled for rendering, and both the features and images are warped from one to the other to calculate the reprojection loss.
GeoD~\cite{geod} tackles the problem by making the discriminator 3D-aware. A geometry branch and a consistency branch are added to the discriminator to extract shapes and evaluate consistency from the generator's outputs and in turn, supervise the generator.

To generate 3D-aware images on larger resolutions efficiently, a variety of methods operate neural fields in a small resolution and leverage convolutional neural networks for upsampling the image/features to a higher resolution.
StyleNeRF~\cite{stylenerf} integrates the neural fields into a style-based generator. The low-resolution NeRF outputs features rather than colors which are further processed by convolutional layers.
StyleSDF~\cite{stylesdf} merges a signed distance function-based representation into neural fields. The output features from the neural fields are passed to a style-based 2D generator for high-resolution generation. Two discriminators operate on the neural field and the 2D generator separately.
CIPS-3D~\cite{cips3d} uses a shallow NeRF network to get the features and densities of all points. A deep implicit neural representation network then predicts the color of each pixel independently based on the feature vector of that pixel. Each network is accompanied by a discriminator.
Despite the high-resolution images of high fidelity achieved, introducing convolutional layers for 2D upsampling may harm the 3D consistency. Carefully designed architectures and regularizers are necessary to mitigate the problem.
StyleNeRF~\cite{stylenerf} uses a well-thought-out upsampler based on 1x1 convolutional kernels. Moreover, a NeRF path regularizer is designed to force the output of CNNs to be similar to the output of NeRF.
GRAM-HD~\cite{xiang2022gramhd} designs a super-resolution module that upsamples the manifold to a higher resolution. Images are rendered from upsampled manifolds.
EpiGRAF~\cite{epigraf} bypasses the use of convolutional neural networks and instead operates directly on the output of a high-resolution neural field. It achieves this by introducing a patch-based discriminator that is modulated by the patch location and scale parameters.

Regarding camera poses, most methods assume a prior distribution from the dataset. 
Several methods\cite{gram,eg3d,xiang2022gramhd,epigraf,schwarz2022voxgraf}, however, leverage ground-truth poses of the dataset for sampling and training, resulting in a significant improvement in the quality of both the images and geometry. This demonstrates the importance of having accurate camera distribution. CAMPARI~\cite{campari} attempts to learn the pose distribution automatically from datasets and leverages a camera generator to learn the distribution shift based on a prior distribution. However, the results are sensitive to the prior initialization.
PoF3D~\cite{shi2023pof3d}, in contrast, infers the camera poses from the latent code and frees the model from prior knowledge. Besides, a pose-aware discriminator is designed to facilitate pose learning on the generator side.

With the advent of generative neural fields, researchers also explore compositional generation. 
GSN~\cite{GSN} decomposes global neural radiance fields into several local neural radiance fields to model parts of the whole scene.
GIRAFFE~\cite{giraffe} and GIRAFFE-HD~\cite{xue2022giraffehd} represent scenes as compositional generative neural radiance fields, allowing the independent control over multiple foreground objects as well as the background.
DisCoScene~\cite{xu2022discoscene} also proposes compositional generation but introduces scene layout prior to better disentangle and model the scene. 
UrbanGIRAFFE~\cite{yang2023urbangiraffe} further leverages panoptic layout prior to additionally enabling control over large camera movement and background semantics.

Besides, editing and controllability in the generation process have sparked the interest of researchers.
A few works focus on semantic control in 3D generation.
\cite{semanticguidedhuman} generates a semantic map from generative radiance fields conditioned on a semantic code as well as the sampled human pose and camera pose. It then employs an encoder-decoder structure to synthesize a human image based on the semantic map and a sampled texture latent code. The content can be manipulated by interpolating codes and sampling different poses.
FENeRF~\cite{fenerf} and IDE-3D~\cite{sun2022ide} render semantic maps and color images from generative neural fields simultaneously. The semantic maps can be used to edit the 3D neural fields via GAN inversion techniques~\cite{image2stylegan,alae}.
Pix2NeRF~\cite{cai2022pix2nerf} employs generative models to translate a single input image to radiance fields, granting control in the 3D space (\textit{e.g.}, changing viewpoints). To accomplish this, an encoder is added to the GAN framework to convert the input to the latent space, thereby establishing a reconstruction objective for learning. 
D3D~\cite{tewari2022disentangled3d} decomposes the generation into two distinct components: shape and appearance. This decomposition allows for independent control over geometry and color, respectively.
3D-GIF~\cite{3DGIF} and VoLux-GAN~\cite{tan2022volux} seek control over lights.
3D-GIF explicitly predicts the albedo, normal, and specular coefficients for each point. To synthesize an image that takes lighting into account, it employs volume rendering and photometric image rendering techniques using sampled lighting sources. 
VoLux-GAN also predicts albedos, normals, diffuse components, and specular components with the neural fields but instead uses an HDR environmental map to model the lighting. This approach enables VoLux-GAN to achieve high dynamic range imaging (HDRI) relighting capabilities.

In addition to GAN-based methods, NeRF-VAE~\cite{nerfvae} leverages a variational autoencoder~\cite{vae} to model the distribution of radiance fields. The model takes a set of images and their corresponding camera poses from the same scene as input and generates a latent variable. The latent variable serves as input for the generator to synthesize the content. Next, a reconstructed image is obtained by volume rendering the synthesized content using the input camera poses. The reconstructed images are expected to be similar to the input images.
LOLNeRF~\cite{Rebain2022CVPR} employs an auto-decoder to learn a 3D generative model, where pixel-level supervision can be applied in contrast to image-level supervision used in GAN-based methods.


\subsection{Hybrid Representations}

Implicit representations can effectively optimize the entire 3D shape based on 2D multi-view observations through differentiable rendering. 
As a result, many studies~\cite{graf,pigan,giraffe,stylenerf,Gao2022NeurIPS} opt to integrate implicit representations into the generator to achieve 3D-aware image synthesis using 2D supervision.
Implicit representations implemented by MLPs are memory-efficient but tend to have a long evaluation time. 
On the other hand, explicit representations like voxel grids and depth work effectively with CNNs and are efficient for high-resolution image rendering. However, they suffer from memory overhead and view consistency issues.
By combining implicit and explicit representations, their complementary benefits can be harnessed for 3D-aware image synthesis, potentially enhancing image quality and rendering efficiency, which is in line with the results from the benchmark by Wang \etal~\cite{wang2023benchmarking}.

 


VolumeGAN~\cite{xu2021volumegan} proposes to represent objects using structural and textural representations.
To capture the structure, they first construct a feature volume and then utilize the features queried within this volume, along with the raw coordinates, to learn generative implicit feature fields.
Additionally, a texture network similar to StyleGAN2 is employed to provide texture information to the feature fields. 
By utilizing explicit voxel grids and implicit feature fields, VolumeGAN enhances both the evaluation speed and the quality of synthetic images. 
However, it is challenging to improve the resolution of structural representation because a larger feature volume results in an increased computational burden.
Unlike VolumeGAN, EG3D~\cite{eg3d} introduces the use of tri-planes as explicit representations instead of voxels. 
EG3D adopts a 2D generator to generate the tri-planes, offering a computationally efficient approach to scale up to high resolutions. 
Besides, EG3D renders a low-resolution feature map that is upsampled to the target resolution using a neural renderer, i.e., a 2D CNN, further reducing the computational burden of the volume rendering.
Moreover, EG3D incorporates additional techniques, such as generator pose conditioning and dual discrimination, to address view inconsistencies.
Another approach, Next3D~\cite{sun2022next3d}, proposes the combination of explicit mesh-guided control and implicit volumetric representation, aiming to leverage the benefits of both controllability and quality.


Recently, a few works have started exploring diffusion models for 3D generation.
GAUDI~\cite{bautista2022gaudi} utilizes a latent representation that can be decoded into triplane features and camera poses for rendering. They then train a diffusion model on this latent space.
RenderDiffusion~\cite{anciukevivcius2022renderdiffusion} replaces U-Net, a common structure used in diffusion models, with a tri-plane feature-based network for denoising. This allows for learning 3D generation solely from 2D supervision.

It has been shown that hybrid representations are effective in producing high-quality 3D-aware images and 3D shapes.
As a result, subsequent works such as AvatarGen~\cite{zhang2022avatargen} and GNARF~\cite{ Bergman2022ARXIV} also adopt tri-plane representations for human synthesis.
However, there is still room for improvement,  particularly in terms of training speed and strategy. %
For instance, VolumeGAN relies on progressive training, which presents challenges when transitioning to another framework.






==> sections/06_applications.tex <==

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/app_giraffe.jpg}\\
  \vspace{-0.1cm}
  Layout editing 
  \includegraphics[width=\linewidth]{figures/app_voluxgan.jpg}\\
  \vspace{-0.1cm}
  Relighting
  \includegraphics[width=\linewidth]{figures/app_ide3d.jpg}\\
  \vspace{-0.1cm}
  Semantic Editing
  \includegraphics[width=\linewidth]{figures/app_autosdf.jpg}\\
  \vspace{-0.1cm}
  Reconstruction
\caption{\textbf{Applications}. 3D generative models have enabled various applications in editing, reconstruction, and representation learning. Images adapted from \cite{giraffe}\cite{tan2022volux}\cite{sun2022ide},\cite{mittal2022autosdf}. }
\label{fig:applications}
\end{figure}

\section{Applications}\label{sec:applications}

The emergence of 3D generative models has facilitated numerous promising applications, as shown in \cref{fig:applications}. In this section, we delve into the various applications of 3D generative models, specifically focusing on editing, reconstruction, and representation learning. Editing is further categorized into two distinct types: shape editing and 3D-aware image editing. This categorization is based on whether the resulting output exists in a 3D or 2D space.


\subsection{3D Shape Editing}\label{sec:shape_editing}


Several classical methods are available for 3D shape editing, including skeleton-based deformation and cage-based deformation. We refer to \cite{Yuan2021JCST} for a detailed survey of classical shape editing methods. Here, our focus lies on shape editing methods that apply to 3D   generative models.




\noindent\textbf{3D space editing: } Several works edit shapes relying on user manipulation in the 3D shape space. Liu et al.~\cite{Liu2017TDV} propose a method where users paint 3D shapes using voxel grids, which are then refined using a 3D GAN. Li et al.~\cite{li2020learning} allow users to edit a part of the voxel grid and automatically
deform and re-assemble all parts into a plausible shape. Alternatively, a few methods study shape editing controlled by more compact representations, such as sparse 3D points or bounding boxes~\cite{hao2020dualsdf,deng2021deformed,ibing20213d,Zheng2021CVPR}. While the aforementioned methods focus on editing rigid shapes, gDNA~\cite{gdna} enables reposing articulated human bodies controlled by human skeletons. 

\noindent\textbf{Latent code editing: } Another set of methods updates the latent space of the generative model without requiring user manipulation in the 3D space. Part-aware generative models that assign a latent code to each part inherently possess the ability of fine-grained part-level  control~\cite{gal2020mrgan,li2021sp}. Furthermore,
several methods explore shape editing guided by semantic labels or language descriptions~\cite{Jahan2021CGF,Liu2022CVPR,Fu2022ARXIV}. 



\subsection{3D-Aware Image Editing}\label{sec:image_editing}
We refer to 3D-aware image editing as the technique that produces an edited 2D image as the outcome. We divide 3D-aware image editing methods into two categories: one that edits a set of physically meaningful 3D factors, while the other manipulates the latent code without explicit physical meaning.

\noindent\textbf{Physical factor editing: }
All 3D-aware image synthesis methods allow users to control camera poses, resulting in 2D images from various viewpoints~\cite{graf,pigan,gram,stylenerf,stylesdf,eg3d}. In addition to camera poses, several methods~\cite{nguyen2020blockgan,Liao2020CVPR,giraffe} enable the editing of object poses and the insertion of new objects by modeling the compositional nature of the scene. The study of re-lighting is also conducted through the disentangling of the albedo, normal, and specular coefficients~\cite{generativeoccupancy,3DGIF,tan2022volux}. More recently, several generative models for neural articulated radiance fields are proposed for human bodies~\cite{noguchi2022unsupervised,Bergman2022ARXIV,zhang2022avatargen}, enabling shape manipulation driven by human skeletons. 

\noindent\textbf{Latent code editing: }
The latent code captures all the other variations that are not represented by the physically meaningful 3D factors, e.g., object shape and appearance. One line of work involves editing the global attributes of the generated content. Several methods learn disentangled shape and appearance code for generative radiance fields, enabling independent interpolation of shape and appearance~\cite{graf,tewari2022disentangled3d}. CLIP-NeRF~\cite{Wang2022CVPR} further allows for controlling the shape and appearance of generative radiance fields using language or a guidance image. Another line of work explores more fine-grained local editing through semantic manipulation. FENeRF~\cite{fenerf} and IDE-3D~\cite{sun2022ide} allow users to edit the semantic masks and generate edited 3D-aware images accordingly.


\subsection{3D Reconstruction}

Two common approaches exist for utilizing 3D generative models in reconstruction, depending on whether test-time optimization is employed or not.

\noindent\textbf{Armotized inference:} 
Generative models equipped with an encoder, such as VAE, offer a natural means of reconstructing 3D shapes from a given input. In contrast to standard 3D reconstruction focusing on one-to-one mapping from the input to the target 3D shape, generative methods allow for sampling numerous possible shapes from the posterior distribution. This line of work is applicable to different types of input by simply switching the encoder. Common input choices are single-view image~\cite{Zhang2022ARXIV,mittal2022autosdf} and point cloud~\cite{Zhang2022ARXIV}.

\noindent\textbf{Model inversion:} 
Another line of methods leverages the inversion of generative models for reconstruction, typically requiring test-time optimization. By adopting an auto-decoder framework, a complete shape can be reconstructed from a partial observation via  optimizing the latent code to align with the partial observation\cite{deepsdf,Duggal2021ARXIV}.

While the aforementioned methods rely on 3D supervision, recent advancements demonstrate single-view image-based 3D reconstruction by inverting the 3D-aware image generative models using only 2D supervision~\cite{pigan,eg3d}. This approach aligns with the classical concept of Analysis by Synthesis~\cite{Vuille2006Vision}. Notably, by inverting 3D-aware image generation models, it becomes possible to recover camera poses, thereby enabling category-level object pose estimation~\cite{Chen2020ECCV,Guo2022ECCV,shi2023pof3d}.



\subsection{Representation Learning}

Another common application of generative models is to learn better representations for downstream tasks, e.g., classification or segmentation.
Notably, representation learning on point clouds has proven effective for tasks like model classification and semantic segmentation~\cite{achlioptas2018learning,Eckart2021CVPR,xie2021generative}. Similarly, generative models of voxel grids have been adopted for tasks such as model classification, shape recovery, and super-resolution~\cite{xie2020generative}.









==> tables/method_summary.tex <==

\begin{table*}[t]
\centering
\caption{\textbf{Properties of representative 3D generative models.} Units for ``FLOPS" and ``\#Params." are in G and M, respectively. We calculate the two metrics for methods implemented using a PyTorch~\cite{NEURIPS2019pytorch} implementation. }
\label{tab:properties}

\begin{subtable}{0.49\textwidth}
\caption{Methods using 3D supervision.}
\label{tab:shape_generation}
\centering\fontsize{6pt}{6pt}\selectfont
\SetTblrInner{rowsep=3.0pt}       %
\SetTblrInner{colsep=3.5pt}       %
\begin{tblr}{
    cells={halign=c,valign=m},  %
    hline{1,2,15}={1-5}{},   %
    hline{1,15}={1.0pt},        %
    hline{2}={0.7pt},           %
    row{odd} = {gray!0}, 
    row{even} = {gray!5},
}
\textbf{Method} & \textbf{3D Representation} & \textbf{FLOPS} & \textbf{\#Params.} & \textbf{Shape Resolution}\\
PQ-Net~\cite{wu2020pq} 
& Voxel grid
& 0.02
& 13.62
& $64\times64\times64$
\\
AutoSDF~\cite{mittal2022autosdf} 
& Voxel grid
& 997.41
& 2941.10
& $64\times64\times64$
\\
PointFlow~\cite{yang2019pointflow} 
& Point cloud 
& 105.89
& 1.06
& 2048
\\
Hui~\etal~\cite{hui2020progressive} 
& Point cloud 
& 25.79
& 12.71
& 2048
\\
ShapeGF~\cite{cai2020learning} 
& Point cloud 
& 413.85
& 4.17
& 2048
\\
SoftFlow~\cite{kim2020softflow} 
& Point cloud 
& 5.26
& 6.50
& 2048
\\
SP-GAN~\cite{li2021sp} 
& Point cloud 
& 1.64
& 0.59
& 2048
\\
Generative PointNet~\cite{xie2021generative} 
& Point cloud 
& 91.86
& 1.39
& 2048
\\
Luo~\etal~\cite{luo2021diffusion} 
& Point cloud 
& 67.33
& 3.30
& 2048
\\
IM-Net~\cite{chen2019learning} 
& Neural field
& 799.70
& 3.05
& $256 \times 256 \times 256$
\\
Deng~\etal~\cite{deng2021deformed} 
& Neural field 
& 209.11
& 0.10
& $256 \times 256 \times 256$ 
\\
gDNA~\cite{chen2022gdna} 
& Neural field 
& 425.90
& 0.87
& $256 \times 256 \times 256$
\\
ShapeAssembly~\cite{jones2020shapeassembly} 
& Program 
& 0.02
& 1.41
& -  
\end{tblr}
\end{subtable}
\hfill
\begin{subtable}{0.49\textwidth}
\caption{Methods using 2D supervision.}
\label{tab:3dimage_generation}
\centering\fontsize{6pt}{6pt}\selectfont
\SetTblrInner{rowsep=3.0pt}       %
\SetTblrInner{colsep=4.8pt}       %
\begin{tblr}{
    cells={halign=c,valign=m},  %
    hline{1,2,15}={1-5}{},   %
    hline{1,15}={1.0pt},        %
    hline{2}={0.7pt},           %
    row{odd} = {gray!0}, 
    row{even} = {gray!5},
}
\textbf{Method}  & \textbf{3D Representation} & \textbf{FLOPS} & \textbf{\#Params.} & \textbf{Image Resolution} \\
Shi~\etal~\cite{shi20223d}
& Depth map
& 63.24
& 55.81
& $256 \times 256$
\\
Schwarz~\etal~\cite{graf}
& Neural field
& 177.03
& 0.68
& $64 \times 64$
\\
Niemeyer~\etal~\cite{giraffe}
& Neural field
& 5.21
& 0.75
& $256 \times 256$
\\
Chan~\etal~\cite{pigan}
& Neural field
& 842.42
& 1.91
& $256 \times 256$
\\
Pan~\etal~\cite{shadegan}
& Neural field
& 1243.66
& 1.91
& $256 \times 256$
\\
Niemeyer~\etal~\cite{campari}
& Neural field
& 183.86
& 0.36
& 128 $\times$ 128
\\
Xu~\etal~\cite{generativeoccupancy}
& Neural field
& 621.53
& 1.91
& $256 \times 256$
\\
Sun~\etal~\cite{fenerf}
& Neural field
& 2094.73
& 2.70
& 256 $\times$ 256
\\
StyleNeRF~\cite{stylenerf}
& Neural field
& 13.49
& 7.63
& $1024 \times 1024$
\\
GRAM~\cite{gram}
& Neural field
& 977.91
& 1.95
& $256 \times 256$
\\
GIRAFFE HD~\cite{xue2022giraffehd}
& Neural field
& 35366.12
& 12.78
& 1024 $\times$ 1024
\\
VolumeGAN~\cite{xu2021volumegan}
& Hybrid
& 32.52
& 8.67
& $256 \times 256$
\\
EG3D~\cite{eg3d}
& Hybrid
& 25.78
& 30.60
& 512$\times$512
\end{tblr}
\end{subtable}

\end{table*}










==> tables/representation_classification.tex <==
  



 
\begin{table*}
    \centering\scriptsize
    \SetTblrInner{rowsep=1.0pt}       %
    \SetTblrInner{colsep=1.5pt}       %
    \caption{%
        \textbf{Representative 3D generative models categorized by supervision and 3D representation.}
        Methods in \com{green} model 3D representation in a compositional way.
        \gloseman{Orange} denotes that the method supports controllability through semantic maps, while those in \gloreli{pink} support relighting.
        Methods in \glohuman{blue} enable control through human pose.
        Note that generative models, such as energy-based models and normalizing flows, are not included as this table focuses on the most frequently used types of 3D generative models (GANs, VAEs, and Diffusion Models).
    }
    \label{tab:representation_classification}
    \begin{tblr}{
        cells={halign=c,valign=m},  %
        cell{1}{1}={r=2}{},         %
        cell{1}{2}={r=2}{},         %
        cell{1}{3}={c=3}{},         %
        cell{3}{1}={r=4}{},         %
        cell{7}{1}={r=4}{},
        hline{2}={3-5}{},
        hline{1,3,7,11}={1-5}{},
        hline{4,5,6,8,9,10}={2-5}{},   %
        vline{1,2,3,6}={1-10}{},      %
        vline{4,5}={2-10}{},      %
        column{3}={7.85cm},
        column{4}={2.4cm},
        column{5}={3.5cm},
    }
     \textbf{Supervision} & \textbf{3D Representation} & \textbf{Generative Model}    &               &    \\
                 &                   &  \textbf{GAN}               & \textbf{VAE}           & \textbf{Diffusion} \\
3D   & Point Clouds      & \glo{Achlioptas \etal\cite{achlioptas2018learning}}, \glo{Shu \etal\cite{shu20193d}}, \glo{Valsesia \etal\cite{valsesia2018learning}}, \glo{Spectral-GAN\cite{ramasinghe2020spectral}}, \glo{Hui \etal\cite{hui2020progressive}}, \glo{Arshad \etal\cite{arshad2020progressive}}, \com{SP-GAN\cite{li2021sp}}, \com{MRGAN\cite{gal2020mrgan}} & \glo{Zamorski \etal\cite{zamorski2020adversarial}} & \glo{ShapeGF\cite{cai2020learning}}, \glo{Luo \etal\cite{ luo2021diffusion}}, \glo{PVD\cite{zhou20213d}}, \glo{lion\cite{zeng2022lion}}, \glo{PSF\cite{wu2022fast}} \\
                 & Voxel Grids       & \glo{Wu \etal\cite{wu2016learning}}, \glo{Ibing \etal\cite{ibing2021octree}},\com{SAGNet\cite{wu2019sagnet}}, \com{PQ-Net\cite{wu2020pq}}, \com{PAGENet\cite{li2020learning}} & \glo{AutoSDF\cite{mittal2022autosdf}}, \glo{Brock \etal\cite{brock2016generative}} & \glo{DiffRF\cite{muller2023diffrf}} \\
                 & Neural Fields     & \glo{IM-Net\cite{chen2019learning}}, \glo{Kleineberg \etal\cite{kleineberg2020adversarial}}, \glo{Ibing \etal\cite{ibing20213d}}, \glo{gDNA\cite{gdna}}, \glo{SurfGen\cite{surfgen}} & - & \glo{Dupont \etal\cite{dupont2022data}},  \glo{Diffusion-SDF\cite{chou2022diffusionsdf}}, \glo{3D-LDM\cite{nam20223d}}, \glo{Rodin\cite{wang2022rodin}}, \glo{Shue \etal\cite{shue20223d}} \\
                 & Mesh              & \glo{Ben-Hamu \etal\cite{ben2018multi}} & \glo{TM-Net\cite{gao2021tm}}, \glo{SDM-NET\cite{gao2019sdm}} & \glo{MeshDiffusion\cite{liu2023meshdiffusion}}, \glo{SLIDE\cite{lyu2023controllable}} \\
2D   & Depth/Normal Maps & \glo{S$^2$-GAN\cite{wang2016generative}}, \glo{RGBDGAN\cite{noguchi2019rgbd}}, \glo{DepthGAN\cite{shi20223d}} & - & - \\
                 & Voxel Grids       & \glo{VoxGRAF\cite{schwarz2022voxgraf}}, \glo{HoloGAN\cite{nguyen2019hologan}}, \glo{VON\cite{zhu2018visual}},  \glo{NGP\cite{chen2021towards}},\glo{PLATONICGAN\cite{Henzler2019ICCV}}, \com{BlockGAN\cite{nguyen2020blockgan}} & - & - \\
                 & Neural Fields     & \glo{GRAF\cite{graf}}, \glo{$\pi$-GAN\cite{pigan}}, \glo{CAMPARI\cite{campari}}, \glo{CIPS-3D\cite{cips3d}}, \glo{GOF\cite{generativeoccupancy}}, \glo{StyleNeRF\cite{stylenerf}}, \glo{StyleSDF\cite{stylesdf}}, \glo{GRAM\cite{gram}}, \glo{MVCGAN\cite{zhang2022multiview}}, \glo{GeoD\cite{geod}}, \glo{GRAM-HD\cite{xiang2022gramhd}}, \glo{EpiGRAF\cite{epigraf}}, \glo{PoF3D\cite{shi2023pof3d}}, \glo{GSN\cite{GSN}}, \glo{Pix2NeRF\cite{cai2022pix2nerf}}, \glo{Disentangled3D\cite{tewari2022disentangled3d}}, \glo{3D-GIF\cite{3DGIF}}, \glo{NeRF-VAE\cite{nerfvae}}, \glo{LOLNeRF\cite{Rebain2022CVPR}}, \com{DisCoScene\cite{xu2022discoscene}}, \com{GIRAFFE\cite{giraffe}}, \com{GIRAFFE HD\cite{xue2022giraffehd}}, \gloreli{ShadeGAN\cite{shadegan}}, \gloreli{Volux-GAN\cite{tan2022volux}}, \glohuman{3D-SGAN\cite{semanticguidedhuman}}, \gloseman{FENeRF\cite{fenerf}}, \gloseman{IDE-3D\cite{sun2022ide}}& - & -\\
                 & Hybrid           & \glo{EG3D\cite{eg3d}}, \glo{VolumeGAN\cite{xu2021volumegan}}, \glo{Next3D\cite{sun2022next3d}} & - & \glo{GAUDI\cite{bautista2022gaudi}}, \glo{RenderDiffusion\cite{anciukevivcius2022renderdiffusion}} \\
    \end{tblr}
    \vspace{-5pt}
\end{table*}





==> tables/representation_comparison.tex <==

\begin{table*}
    \centering
    \SetTblrInner{rowsep=3pt}       %
    \SetTblrInner{colsep=5pt}       %
    \caption{%
        \textbf{Comparison of different representations} with regard to time efficiency, memory efficiency, representation capability, and NN (neural network) compatibility. A larger number of stars indicates better performance.
    }
    \label{tab:representation_comparison}
    \begin{tblr}{
        cells={halign=c,valign=m},  %
        hline{1,2,6}={1-7}{},   %
        hline{1,6}={1.0pt},        %
        hline{2}={0.7pt},           %
        vline{2,3,4,5,6,7}={1-5}{},      %
    }
        \textbf{3D Representation}  & \raisebox{-.15\height}{\includegraphics[width=0.3cm]{figures/icon/points.png}}\textbf{Point Clouds}  & \raisebox{-.15\height}{\includegraphics[width=0.3cm]{figures/icon/voxel.png}}\textbf{Voxel Grids}   & \raisebox{-.15\height}{\includegraphics[width=0.3cm]{figures/icon/depth.png}}\textbf{Depth/Normal Maps} & \raisebox{-.15\height}{\includegraphics[width=0.3cm]{figures/icon/neural_fields.png}}\textbf{Neural Fields} & \raisebox{-.15\height}{\includegraphics[width=0.3cm]{figures/icon/mesh.png}}\textbf{Mesh}  & \raisebox{-.15\height}{\includegraphics[width=0.3cm]{figures/icon/hybrid.png}}\textbf{Hybrid} \\
        Time Efficiency   & $\star\star\star$           & $\star$             & $\star\star\star\star\star$             &   $\star$          & $\star\star\star\ \star$  & $\star\star\star$   \\
  Memory Efficiency & $\star\ \star$            & $\star\ \star$            & $\star\star\star\ \star$              &   $\star\star\star\star\star$       & $\star\star\star$   & $\star\star\star$\\
  Representation Capability&  $\star\star\star$   & $\star\ \star$            &   $\star$               &     $\star\star\star\star\star$     & $\star\star\star\ \star$  &  $\star\star\star\star\star$  \\
  NN Compatibility & $\star\ \star$             & $\star\star\star\star\star$         & $\star\star\star\star\star$             &   $\star\star\star\star\star$       & $\star$     & $\star\star\star\star\star$ \\
    \end{tblr}
\end{table*}
